Blazar classification from multi-wavelength data using Deep Learning

The Fermi Large Area Telescope (Fermi-LAT) has detected more than 7,000 gamma-ray sources, a significant fraction of which are identified as blazars, while a comparable number remain classified as blazars of uncertain type (BCUs) or are unassociated with counterparts at other wavelengths. The absence of complete multi-wavelength spectral information presents a major obstacle to robust source classification, despite such data providing the most reliable means of understanding blazar properties. In this work, we focus on classifying BCUs into the two primary blazar subclasses, flat-spectrum radio quasars (FSRQs) and BL Lacertae objects (BL Lacs), using a feed-forward artificial neural network (ANN) trained on multi-wavelength observational parameters. We first identify the most informative features by quantifying their information content and then use these features to train the ANN, whose performance is evaluated using a k-fold cross-validation strategy to ensure robust generalization. The trained model is subsequently applied to classify BCUs into BL Lacs and FSRQs. Our results demonstrate that machine learning-based classification using a carefully selected set of multi-wavelength parameters offers an efficient and reliable approach for resolving the nature of BCUs and improving the completeness of the gamma-ray blazar population in Fermi-LAT catalogs.

==> hyperparameter.tex <==
\saqlain{
\subsection{Hyperparameter Optimization}

To maximize the predictive performance of the neural network and mitigate the risk of manual tuning bias, we performed an automated hyperparameter optimization using the Optuna framework. We employed the Tree-structured Parzen Estimator (TPE) algorithm to efficiently explore the hyperparameter search space. This Bayesian optimization method models the probability of a hyperparameter configuration yielding a high validation accuracy, allowing the search to converge significantly faster than random or grid search methods.

The objective of the optimization was to maximize the validation accuracy by minimizing the regularized Cross-Entropy loss $\mathcal{L}(\boldsymbol{\theta})$ for a given batch of $N$ samples. This objective function incorporates the $L_2$ regularization (weight decay) to penalize complex models and prevent overfitting:

\begin{equation}
    \mathcal{L}(\boldsymbol{\theta}) = - \frac{1}{N} \sum_{i=1}^{N} \sum_{c=1}^{C} y_{i,c} \log(\hat{y}_{i,c}) + \frac{\lambda}{2} \|\boldsymbol{\theta}\|_2^2
\end{equation}

\noindent where $C=2$ is the number of classes, $y_{i,c}$ is the binary indicator (0 or 1) for class $c$ in sample $i$, $\hat{y}_{i,c}$ is the predicted probability, $\boldsymbol{\theta}$ represents the model weights, and $\lambda$ is the weight decay hyperparameter being optimized.

The optimization process spanned 50 trials, exploring a mixed search space of continuous, integer, and categorical parameters. The specific hyperparameters tuned included the number of neurons in the first hidden layer ($N_{L1} \in [8, 64]$) and second hidden layer ($N_{L2} \in [4, 32]$), the learning rate ($\eta \in [10^{-5}, 10^{-2}]$), the $L_2$ weight decay ($\lambda \in [10^{-6}, 10^{-3}]$), the dropout probability ($p \in [0.0, 0.5]$), and the batch size ($B \in \{16, 32, 64\}$). To accelerate the search, we utilized an automated pruning strategy (Median Pruner) to terminate unpromising trials early based on intermediate validation accuracy.

The best-performing configuration achieved a validation accuracy of 97.47\%. The resulting optimal architecture consists of 22 neurons in the first hidden layer and 31 neurons in the second. The optimization selected a learning rate of $\eta \approx 4.84 \times 10^{-3}$. Notably, the model preferred a smaller batch size of 16 and minimal regularization, with a weight decay of $\lambda \approx 2.50 \times 10^{-5}$ and a low dropout rate of $p \approx 0.013$. This suggests that the stochastic noise from smaller batch sizes provided sufficient regularization, allowing the model to fit the data efficiently without aggressive weight penalties. The optimal hyperparameters (summarized in Table \ref{tab:hyperparams}) were fixed for the final model training.

\begin{table}[htbp!]
\centering
\caption{Optimal Hyperparameters yielded by Bayesian Optimization (TPE).}
\label{tab:hyperparams}
\begin{tabular}{lcc}
\hline
\textbf{Hyperparameter} & \textbf{Search Space} & \textbf{Optimal Value} \\ \hline
Neurons (Layer 1) & $[8, 64]$ & 22 \\
Neurons (Layer 2) & $[4, 32]$ & 31 \\
Learning Rate ($\eta$) & $[10^{-5}, 10^{-2}]$ & $4.84 \times 10^{-3}$ \\
Weight Decay ($\lambda$) & $[10^{-6}, 10^{-3}]$ & $2.50 \times 10^{-5}$ \\
Dropout Rate ($p$) & $[0.0, 0.5]$ & 0.013 \\
Batch Size ($B$) & $\{16, 32, 64\}$ & 16 \\ \hline
\textbf{Best Accuracy} & - & \textbf{97.47\%} \\ \hline
\end{tabular}
\end{table}
}
